TEDRA: Text-based Editing of Dynamic and Photoreal Actors

Over the past years, significant progress has been made in creating photorealistic and drivable 3D avatars solely from videos of real humans. However, a core remaining challenge is the fine-grained and user-friendly editing of clothing styles by means of textual descriptions. To this end, we present TEDRA, the first method allowing text-based edits of an avatar, which maintains the avatar's high fidelity, space-time coherency, as well as dynamics, and enables skeletal pose and view control. We begin by training a model to create a controllable and high-fidelity digital replica of the real actor. Next, we personalize a pretrained generative diffusion model by fine-tuning it on various frames of the real character captured from different camera angles, ensuring the digital representation faithfully captures the dynamics and movements of the real person. This two-stage process lays the foundation for our approach to dynamic human avatar editing. Utilizing this personalized diffusion model, we modify the dynamic avatar based on a provided text prompt using our Personalized Normal Aligned Score Distillation Sampling (PNA-SDS) within a model-based guidance framework. Additionally, we propose a time step annealing strategy to ensure high-quality edits. Our results demonstrate a clear improvement over prior work in functionality and visual quality.

==> tables/rebuttal_fid.tex <==
\begin{table}[htbp]
    \tiny
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{} & \textbf{Ours} & \textbf{InstructN2N}& \textbf{AvatarStudio}  \\
        \hline
        FID & \textbf{0.2098}& 0.1656 & 0.1412\\
    \hline
    \end{tabular}
    \caption{The FID scores.}
    \label{tab:rebutallfid}
\end{table}
